Invariance and the knot Floer cube of resolutions

This paper considers the invariance of knot Floer homology in a purely algebraic setting, without reference to Heegaard diagrams, holomorphic disks, or grid diagrams. We show that (a small modification of) Ozsv\'ath and Szab\'o's cube of resolutions for knot Floer homology, which is assigned to a braid presentation with a basepoint, is invariant under braid-like Reidemeister moves II and III and under conjugation. All moves are assumed to happen away from the basepoint. We also describe the behavior of the cube of resolutions under stabilization. The techniques echo those employed to prove the invariance of HOMFLY-PT homology by Khovanov and Rozansky, and are further evidence of a close relationship between the theories. The key idea is to prove categorified versions of certain equalities satisfied by the Murakami-Ohtsuki-Yamada state model for the HOMFLY-PT polynomial.

==> ellipse.tex <==
\xy
%(0,0);(0,10) **\crv{(2,1) & (4,5) & (2,9)};
%(0,0);(0,10) **\crv{(-2,1) & (-4,5) & (-2,9)};
(0,0)*\xycircle(4,10){};
\endxy

==> halfellipse.tex <==
\xy
%(-3.5,0);(3.5,0) **\crv{(-3,-4) & (-3,-8) & (0,-10) & (3,-8) & (3,-4)};
(-3.5,3);(3.5,3) **\crv{(-3.5,0) & (-3,-4) & (-3,-8) & (0,-10) & (3,-8) & (3,-4) & (3.5,0)};
\endxy

==> reid3000d1.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{000};
\endxy}

==> reid3000d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{000};
\endxy}

==> reid3001d1.tex <==
%001-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmr";"tr"};
{\ar "tmm";"tm"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{001};
\endxy}

==> reid3001d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmr";"tr"};
{\ar "tmm";"tm"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{001};
\endxy}

==> reid3010d1.tex <==
%010-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{010};
\endxy}

==> reid3010d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{010};
\endxy}

==> reid3011d1.tex <==
%011-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tm"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
"vtx3"*{\scriptstyle{\bullet}};
%extra dots and their labels
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
%(5,2.6)*{\scriptstyle{s_2}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{011};
\endxy}

==> reid3011d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tm"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
"vtx3"*{\scriptstyle{\bullet}};
%extra dots and their labels
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
%(5,2.6)*{\scriptstyle{s_2}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{011};
\endxy}

==> reid3100d1.tex <==
%100-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{100};
\endxy}

==> reid3100d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(-5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{100};
\endxy}

==> reid3101d1.tex <==
%101-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{101};
\endxy}

==> reid3101d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-12)*=<25pt,15pt>[F]{101};
\endxy}

==> reid3110d1.tex <==
%110-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(0,-12)*=<25pt,15pt>[F]{110};
\endxy}

==> reid3110d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(-5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(0,-12)*=<25pt,15pt>[F]{110};
\endxy}

==> reid3111d1.tex <==
%111-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar "tmr";"tr"};
{\ar "vtx1";"tl"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"vtx3"};
{\ar@{-} "vtx3";"vtx2"};
{\ar@{-} "vtx2";"vtx1"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "vtx2";"tmr"};
{\ar@{-} "mr";"vtx2"};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(-5,13.5)*{\scriptstyle{1}};
(0,13.5)*{\scriptstyle{2}};
(5,13.5)*{\scriptstyle{3}};
(-5,-7.5)*{\scriptstyle{4}};
(0,-7.5)*{\scriptstyle{5}};
(5,-7.5)*{\scriptstyle{6}};
(1,7)*{\scriptstyle{7}};
(-6,7)*{\scriptstyle{8}};
(1,-1)*{\scriptstyle{9}};
(-7,-1)*{\scriptstyle{10}};
(6.5,5)*{\scriptstyle{11}};
(6.5,0)*{\scriptstyle{12}};
(0,-12)*=<25pt,15pt>[F]{111};
\endxy}

==> reid3111d2.tex <==
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bmr";
(0,-6)*{}="bmm";
(5,-6)*{}="bml";
(-5,0)*{}="mr";
(0,0)*{}="mm";
(5,0)*{}="ml";
(-5,6)*{}="tmr";
(0,6)*{}="tmm";
(5,6)*{}="tml";
(-5,12)*{}="tr";
(0,12)*{}="tm";
(5,12)*{}="tl";
(2.5,9)*{}="vtx1";
(-2.5,3)*{}="vtx2";
(2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar "tmr";"tr"};
{\ar "vtx1";"tl"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"vtx3"};
{\ar@{-} "vtx3";"vtx2"};
{\ar@{-} "vtx2";"vtx1"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "vtx2";"tmr"};
{\ar@{-} "mr";"vtx2"};
(-5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(-5,13.5)*{\scriptstyle{1}};
(0,13.5)*{\scriptstyle{2}};
(5,13.5)*{\scriptstyle{3}};
(-5,-7.5)*{\scriptstyle{4}};
(0,-7.5)*{\scriptstyle{5}};
(5,-7.5)*{\scriptstyle{6}};
(-1,7)*{\scriptstyle{7}};
(6,7)*{\scriptstyle{8}};
(-1,-1)*{\scriptstyle{9}};
(6.5,-1)*{\scriptstyle{10}};
(-7,5)*{\scriptstyle{11}};
(-7,0)*{\scriptstyle{12}};
(0,-12)*=<25pt,15pt>[F]{111};
\endxy}

==> reid3complexes.tex <==
%\documentclass{amsart}
%\usepackage{amssymb,amsmath,amsthm,latexsym} 
%\usepackage{subfigure}
%\usepackage[pdftex]{color,graphicx}
%\usepackage[all]{xy}
%\usepackage{rotating}
%\xyoption{all}
%\xyoption{line}
%\xyoption{knot}
%\xyoption{curve}

%\begin{document}

$$\xymatrix@R-15pt{
%blank
&
%100-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tm"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
"vtx3"*{\scriptstyle{\bullet}};
%extra dots and their labels
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
%(5,2.6)*{\scriptstyle{s_2}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{100};
\endxy}
\ar[r]
\ar[dr]
&
%110-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmr";"tr"};
{\ar "tmm";"tm"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{110};
\endxy}
\ar[dr]
&
%blank
\\
%000-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar "tmr";"tr"};
{\ar "vtx1";"tl"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
{\ar@{-} "bml";"vtx3"};
{\ar@{-} "vtx3";"vtx2"};
{\ar@{-} "vtx2";"vtx1"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "vtx2";"tmr"};
{\ar@{-} "mr";"vtx2"};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{000};
\endxy}
\ar[ur]
\ar[r]
\ar[dr]
&
%010-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"mm"};
{\ar@{-} "bmm";"ml"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx3"*{\scriptstyle{\bullet}};
%(-5,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{010};
\endxy}
\ar[ur]
\ar[dr]
&
%101-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{101};
\endxy}
\ar[r]
&
%111-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tl"};
{\ar "tmm";"tm"};
{\ar "tmr";"tr"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,9)*{\scriptstyle{\bullet}};
%(-7,7)*{\scriptstyle{s_1}};
(0,9)*{\scriptstyle{\bullet}};
%(-2,7)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{111};
\endxy}
\\
%blank
&
%001-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmr"};
{\ar@{-} "mr";"tmm"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
"vtx2"*{\scriptstyle{\bullet}};
%(5,2.6)*{\scriptstyle{s_2}};
(0,-8)*{001};
\endxy}
\ar[ur]
\ar[r]
&
%011-resolution
{\xy
%(-5,-10)*{}="bl";
%(0,-10)*{}="bm";
%(5,-10)*{}="br";
(-5,-6)*{}="bml";
(0,-6)*{}="bmm";
(5,-6)*{}="bmr";
(-5,0)*{}="ml";
(0,0)*{}="mm";
(5,0)*{}="mr";
(-5,6)*{}="tml";
(0,6)*{}="tmm";
(5,6)*{}="tmr";
(-5,12)*{}="tl";
(0,12)*{}="tm";
(5,12)*{}="tr";
(-2.5,9)*{}="vtx1";
(2.5,3)*{}="vtx2";
(-2.5,-3)*{}="vtx3";
{\ar "tml";"tm"};
{\ar@{->} "tmr";"tr"};
{\ar "tmm";"tl"};
{\ar@{-} "ml";"tml"};
{\ar@{-} "mm";"tmm"};
{\ar@{-} "mr";"tmr"};
{\ar@{-} "bml";"ml"};
{\ar@{-} "bmm";"mm"};
{\ar@{-} "bmr";"mr"};
%{\ar@{-} "br";"bmr"};
%{\ar@{-} "bm";"bmm"};
%{\ar@{-} "bl";"bml"};
"vtx1"*{\scriptstyle{\bullet}};
%(-6,7.5)*{\scriptstyle{s_1}};
(0,3)*{\scriptstyle\bullet};
%(-2,2.5)*{\scriptstyle{s_2}};
(5,3)*{\scriptstyle\bullet};
%(7,2.5)*{\scriptstyle{s_2}};
(-5,-3)*{\scriptstyle{\bullet}};
%(-7,-2.5)*{\scriptstyle{s_3}};
(0,-3)*{\scriptstyle{\bullet}};
%(-2,-2.5)*{\scriptstyle{s_3}};
(5,9)*{\scriptstyle{\bullet}};
%(7,6.5)*{\scriptstyle{s_1}};
(-5,3)*{\scriptstyle{\bullet}};
%(-7,2.6)*{\scriptstyle{s_2}};
(5,-3)*{\scriptstyle{\bullet}};
%(7,-2.5)*{\scriptstyle{s_3}};
(0,-8)*{011};
\endxy}
\ar[ur]
&
%blank
}$$
%
%\end{document}                                                           
